Smoothness-Penalized Deconvolution (SPeD) of a Density Estimate

This paper addresses the deconvolution problem of estimating a square-integrable probability density from observations contaminated with additive measurement errors having a known density. The estimator begins with a density estimate of the contaminated observations and minimizes a reconstruction error penalized by an integrated squared $m$-th derivative. Theory for deconvolution has mainly focused on kernel- or wavelet-based techniques, but other methods including spline-based techniques and this smoothness-penalized estimator have been found to outperform kernel methods in simulation studies. This paper fills in some of these gaps by establishing asymptotic guarantees for the smoothness-penalized approach. Consistency is established in mean integrated squared error, and rates of convergence are derived for Gaussian, Cauchy, and Laplace error densities, attaining some lower bounds already in the literature. The assumptions are weak for most results; the estimator can be used with a broader class of error densities than the deconvoluting kernel. Our application example estimates the density of the mean cytotoxicity of certain bacterial isolates under random sampling; this mean cytotoxicity can only be measured experimentally with additive error, leading to the deconvolution problem. We also describe a method for approximating the solution by a cubic spline, which reduces to a quadratic program.

==> msaux.tex <==



==> sections/asymptotics.tex <==
\subsection{Consistency}
\textcolor{red}{Add pointwise results, which I think have similar proofs.}

It will turn out that the second term in Lemma \ref{lem:upper}
vanishes as \(\alpha \to 0\), but clearly for fixed \(\delta_n^2\),
the first term increases as \(\alpha \to 0\). For consistency,
therefore, we need \(\alpha\) to decrease, but slowly enough to
guarantee that the first term vanishes.

\begin{theorem}{(Global consistency)}
\label{theorem:consistency}
 Assume that \(\alpha_n\) is chosen so that \(\delta_n^2/\alpha_n \to
 0\) and \(\alpha_n \to 0\). Then
\[
\lim_{n \to \infty} \EE \| f^{\alpha_n}_n - f\|^2 = 0.
\]
\end{theorem}

\input{proofs/theorem:consistency}

Note that Theorem \ref{theorem:consistency} holds under weak
conditions. We assumed that \(g\) is known, but the only property we
need is that it have a.e. non-vanishing Fourier transform, and the
only assumption on the target density \(f\) is that \(f \in
L_2(\RR)\). All that is required is a consistent estimator \(h_n\) of
\(h\).

\subsection{Rates of Convergence}

In deriving rates of convergence for ill-posed problems, it is assumed
that the solution \(f\) is drawn from a ``source set,'' assuming some
\emph{a priori} degree of smoothness (\cite{engl_regularization_1996},
Section 3.2). In \cite{nair_trade-off_1997} Theorem 5.1 and
\cite{engl_optimal_1985} Theorem 3.5, an abstract version of this
Tikhonov problem is analyzed. It is assumed that the target density
\(f \in \cD(L^*L)\) and \(L^*Lf \in \cR(K^*K)\). This assumption is
rather extreme. Namely, it says that \(f^{(2m)} = g*g*\psi\) for some
\(\psi \in L_2(\RR)\); some consequences are that \(f\) has at least
twice plus \(2m\) as many \(L_2\) derivatives as \(g\), and \(\Var(X)
\geq 2\Var(\varepsilon)\). Nevertheless, if one can make this
assumption on \(f\), it is possible to compute rates of convergence
with no further assumptions on \(g\).

\begin{theorem}{(Rates when \(f\) is very smooth)}
\label{theorem:smoothrates}
Suppose \(f\) has four \(L_2(\RR)\) weak derivatives, and \(f^{(4)} =
g*g*\psi\) for some \(\psi \in L_2(\RR)\). Then for sufficiently small
\(\alpha_n\),
\[
\EE\|f^{\alpha_n}_n - f\|^2 \leq C_1 \delta_n^2/\alpha_n + C_2\alpha_n^2,
\]
and if \(\alpha_n = C_3 \delta^{\frac23}\), then
\[
\EE \|f^{\alpha_n}_n - f\|^2 = O(\delta_n^\frac43).
\]
\end{theorem}
\begin{proof}{(Proof of Theorem \ref{theorem:smoothrates})}
Our task is to find the dependence of \(\|f^\alpha - f\|^2\) on
\(\alpha\). Taking Fourier transforms yields \(\omega^4 \tilde
f(\omega) = \tilde g(\omega)^2 \tilde \psi(\omega)\). Then we have
\begin{equation}\begin{aligned}
\|f^\alpha - f\|^2 &= \frac{1}{2\pi}\|\tilde f^\alpha - \tilde f\|^2\\
&= \frac{1}{2\pi} \int_P  \left [ \frac{\alpha_n \omega^{2m}}{\tilde g(\omega)^2 + \alpha_n \omega^{2m}}\right ]^2 |\tilde f(\omega)|^2 \,d\omega,\\
&= \frac{1}{2\pi} \int_P  \left [ \frac{\alpha_n \omega^{2m}}{\tilde g(\omega)^2 + \alpha_n \omega^{2m}}\right ]^2 |\omega^{-2m}\tilde \psi(\omega)/\tilde g(\omega)^2|^2 \,d\omega,\\
&= \frac{\alpha_n^2}{2\pi} \int_P  \left [ \frac{\tilde g(\omega)^2}{\tilde g(\omega)^2 + \alpha_n \omega^{2m}}\right ]^2 |\tilde \psi(\omega)|^2 \,d\omega\\
&\leq \alpha_n^2 \|\psi\|^2,
\end{aligned}\end{equation}
which, combined with Lemma \ref{lem:upper}, gives the bound with \(C_2 = \|\psi\|^2\).

Note that the upper bound is minimized by \(\alpha_n =
(C_1/2C_2)^\frac13 \delta_n^\frac23\). If we set \(\alpha_n = C_3
\delta_n^\frac23\), the upper bound becomes
\begin{equation}\begin{aligned}
\EE\|f_n - f\|^2 &\leq C_1 C_3 \delta_n^\frac43 + C_2 C_3 \delta_n^\frac43\\
&\leq \max \{C_1, C_2\} C_3 \delta_n^\frac43,
\end{aligned}\end{equation}
from which it follows that
\begin{equation}
\EE \|f_n - f\|^2 = O(\delta_n^\frac43).
\end{equation}
\end{proof}

\begin{cor}\label{cor:smoothrates}
Assume the conditions of Theorem \ref{theorem:smoothrates}, and assume that \(\alpha_n = C\delta_n^\frac23\).\\
If \(h_n\) is a kernel density estimate with optimal choice of bandwidth, then
\begin{equation}
\EE \|f^{\alpha_n}_n - f\|^2 = O(n^{-8/15}).
\end{equation}

\noindent If \(h_n\) is a histogram with optimal choice of bin widths, then
\begin{equation}
\EE \|f^{\alpha_n}_n - f\|^2 = O(n^{-4/9}).
\end{equation}
\end{cor}

\begin{proof}{(Proof of Corollary \ref{cor:smoothrates})}
If \(h_n\) is a kernel density estimate with optimal bandwidth, then
\(\delta_n^2 = \|h_n - h\|^2 = O(n^{-\frac45})\)
(\cite{wand_kernel_1994}, Section 2.5), and the result follows
immediately. Similarly, if \(h_n\) is a histogram with optimal binwidth, then by the same section,
\(\delta_n^2 = \|h_n - h\| = O(n^{-\frac23})\).
\end{proof}

\textcolor{red}{Comment on how it seems backward to make strong assumptions on the unknown \(f\), but weak assumptions on the known \(g\)}

\textcolor{red}{Find some rates under assumptions on \(g\) with weak assumptions on \(f\)!!}

\begin{prop}{(Normal errors, i.)}\label{prop:normalerrorsi}
Assume \(g(x) = (2\pi)^{-1} e^{-x^2/2}\), and assume \(\int |\omega^k \tilde f(\omega)|^2\,d\omega < \infty\), with \(1 \leq k \leq 2m\).
Then
\[
\|f^\alpha - f\|^2 \leq \frac{C}{m^kW(1/(m\alpha^{1/m}))^k} \sim \frac{C}{m^k\log(1/(m\alpha^{1/m}))^k}
\]
where \(W\) is the principal branch of the Lambert \(W\) function, and \(C = \|\omega^k\tilde f(\omega)\|^2/2\pi\).
\end{prop}
\begin{proof}{(Proof of Proposition \ref{prop:normalerrorsi})}
\textcolor{red}{(Refer to relevant summary of facts in Fact \ref{fact:lambertW})}\\
First, note that
\begin{equation}\begin{aligned}
\|f^\alpha - f\|^2 &= (2\pi)^{-1} \|\tilde f^\alpha -\tilde f\|^2\\
&= (2\pi)^{-1} \int \left [ \frac{\alpha \omega^{2m}}{e^{-\omega^2} + \alpha \omega^{2m}} \right ]^2 |\tilde f(\omega)|^2 \,d\omega\\
&= (2\pi)^{-1} \int \left [ \frac{\alpha \omega^{2m-k}}{e^{-\omega^2} + \alpha \omega^{2m}} \right ]^2 |\omega^k\tilde f(\omega)|^2 \,d\omega\\
&\leq C \sup_{\omega} \left [ \frac{\alpha \omega^{2m-k}}{e^{-\omega^2} + \alpha \omega^{2m}} \right ]^2
\end{aligned}\end{equation}
by assumption. Now, we address the value of \(\sup_{\omega} \left [
\frac{\alpha \omega^{2m-k}}{e^{-\omega^2} + \alpha \omega^{2m}} \right
]^2\). Let \(\theta(\omega) = \frac{\alpha
\omega^{2m-k}}{e^{-\omega^2} + \alpha \omega^{2m}}\), and since
\(|\theta(\omega)|\) is even, we will only consider \(\omega > 0\),
and seek \(\sup_{\omega > 0} \theta(\omega).\) To that end, note that
\begin{equation}
  \theta(\omega) \leq \alpha \omega^{2m-k}e^{\omega^2}
  \qquad\text{ and }\qquad
  \theta(\omega) \leq \omega^{-k},
\end{equation}
where the upper bounds are increasing and decreasing, respectively, with \(\omega\). Thus
\[
  \sup_{\omega > 0} \theta(\omega) \leq \omega_0^{-k}
\]
with \(\omega_0\) being where the upper bounds intersect, i.e. \(\omega_0>0\) satisfies
\[
  \alpha \omega_0^{2m-k} e^{\omega_0^2} = \omega_0^{-k}.
\]
Taking \(m\)\textsuperscript{th} roots and rearranging, we find
\begin{equation}
(\omega_0^{2}/m) e^{\omega_0^2/m} = 1/(m\alpha^{1/m}),
\end{equation}
so that
\begin{equation}
  \omega_0^2/m = W(1/(m\alpha^{1/m})),
\end{equation}
whence
\begin{equation}
  \omega_0 = \left ( mW(1/(m\alpha^{1/m})) \right )^{\frac12}.
\end{equation}
Thus we have that
\begin{equation}
  \sup_{\omega > 0} \theta(\omega) \leq \left ( mW(1/(m\alpha^{1/m})) \right )^{-\frac{k}{2}},
\end{equation}
from which it follows that
\begin{equation}
  \sup_{\omega} \left [\frac{\alpha \omega^{2m-k}}{e^{-\omega^2} + \alpha \omega^{2m}} \right]^2 = \sup_{\omega > 0} \theta(\omega)^2 \leq \left ( mW(1/(m\alpha^{1/m})) \right )^{-k},
\end{equation}
giving the result.
\end{proof}

\begin{theorem}{(Normal errors, ii.)}\label{theorem:normalerrorsii}
Assume the conditions of Proposition \ref{prop:normalerrorsi}. There
is a choice of \(\alpha_n \to 0\) for which
\[
\EE\|f_n^\alpha - f\|^2 = O([\log \delta_n^{-1}]^{-k}).
\]
\end{theorem}
\begin{proof}{(Proof of Theorem \ref{theorem:normalerrorsii})}
From Lemma \ref{lem:upper} and Proposition \ref{prop:normalerrorsi}, we have that
\begin{equation}\label{eqn:normalupperbound}
\EE \|f_n^{\alpha_n} - f\|^2 \leq C_1\delta_n^2/\alpha_n + \frac{C_2}{m^kW(1/(m\alpha^{1/m}))^k}
\end{equation}
We will use \(\alpha_n = \delta_n^2 W(\delta_n^{-\frac{2}{k}})^{k}\), which comes from the heuristic that the two summands in the upper bound ought to decrease at the same rate, i.e. by solving
\begin{equation}
  \frac{\delta_n^2}{\alpha_n} = \log(\alpha^{-\frac{1}{m}})^{-k},
\end{equation}
where the \(\log(\cdot)\) is used in lieu of \(W(\cdot)\) as a
simplification justified by the fact that \(\log(x) \sim W(x)\) as \(x
\to \infty\). After solving for \(\alpha_n\), constants are ignored
with wild abandon to yield a simpler \(\alpha_n\).

We show that with the above choice of \(\alpha_n\), the bound in
Equation \ref{eqn:normalupperbound} is asymptotically equivalent to
\(C[\log \delta_n]^{-k}\). Plugging
\(\alpha_n\) into the first term, we get
\begin{equation}\begin{aligned}
C_1 \delta_n^2/\alpha_n &= C_1 W(\delta_n^{-\frac{2}{k}})^{-k}.
\end{aligned}\end{equation}
For the second, we have (equivalences are as \(\alpha_n \to 0\) or \(\delta_n \to 0\))
\begin{equation}\begin{aligned}
\frac{C_2}{m^kW(1/(m\alpha^{1/m}))^k}  &C_2\sim m^{-k}\left [\log(1/(m\alpha^{1/m}))\right ]^{-k}\\
&= C_2\left [\log(m^{-m} \alpha_n^{-1})\right ]^{-k}\\
&= C_2\left [\log(m^{-m} \delta_n^{-2} W(\delta_n^{-\frac{2}{k}})^{-k}) \right ]^{-k}\\
&= C_2\left [ -m\log(m) - 2\log(\delta_n) - k \log( W(\delta_n^{-\frac{2}{k}}))\right ]^{-k}\\
&= C_2\left [ -m\log(m) - 2\log(\delta_n) - k \left \{ -\frac{2}{k} \log (\delta_n) - W(\delta_n^{-\frac{2}{k}}) \right \}\right ]^{-k}\\
&=  \frac{C_2}{\left [-m\log(m)+ k W(\delta_n^{-\frac{2}{k}})  \right ]^k}\\
&\sim C_3W(\delta_n^{-\frac{2}{k}})^{-k}\\
\end{aligned}\end{equation}
The above leads us to
\begin{equation}\begin{aligned}
    C_1\delta_n^2/\alpha_n + \frac{C_2}{m^kW(1/(m\alpha^{1/m}))^k} &= O(W(\delta_n^{-\frac{2}{k}})^{-k})\\
    &=O(\log(\delta_n^{-\frac{2}{k}})^{-k})\\
    &=O(\log(\delta_n^{-1})^{-k})\\
\end{aligned}\end{equation}
giving the result.

\end{proof}

\subsection{Constraining the solution}

We know \emph{a priori} that \(f\) is a probability density function, so we
ought to ensure that our estimate is a probability density function as
well. Consider the set \(\cC = \{v \in L_2(\RR): \int v(t)\,dt = 1, \,
v(t) \geq 0\, \forall t \in \RR\}\); this is the set of
square-integrable probability density functions, and now we can
express this requirement as \(f_n^\alpha \in \cC\). One easy-to-manage
approach is to first solve the unconstrained problem and find an
estimate \(f_n^\alpha \not\in \cC\), and then somehow project this
unconstrained estimate onto \(\cC\).

Define the projection operator \(P_A\) onto a closed, convex set \(A
\subset L_2(\RR)\) by
\begin{equation}
P_Au = \argmin_{v \in A} \|u - v\|.
\end{equation}
In words, \(P_A\) maps \(u\) to the nearest (in \(L_2\)) element of \(A\).

Unfortunately, while \(\cC\) is convex, it is not closed. To see this,
note that the zero function is a limit point of \(\cC\): let \(\psi_n
= \frac1n \ind_{[0,n]}\), and note that \(\|\psi_n - 0\| = \|\psi_n\|
= n^{-\frac12} \to 0\) as \(n \to \infty\). Indeed, any non-negative 
function \(v\) with \(\int v < 1\) is a limit point of \(\cC\). Thus
the infimum may not be attained, and the projection operator \(P_\cC\)
is not well-defined.

Instead, we will need to work with approximations to \(\cC\). Let
\[
\cC_a = \{v \in \cC,\,v(t) = 0\,\,\forall t \not\in[-a,a]\}
\]
be the subset of \(\cC\) of functions with support contained in
\([-a,a]\). 
\begin{prop}\label{prop:cCaclosed}
For fixed \(a\), the set \(\cC_a\) is closed and convex.
\end{prop}
\begin{proof}{(Proof of Proposition \ref{prop:cCaclosed})}
Clearly \(\cC_a\) is convex. To see that it is closed, we must show
that any limit point of \(\cC_a\) is also an element of \(\cC_a\). To
that end, suppose \(\{\psi_n\}\subset \cC_a\) and that there is some
\(\psi \in L_2(\RR)\) with \(\|\psi_n - \psi\| \to 0\). Clearly
\(\psi\) is non-negative and has support contained in \([-a,a]\). We
need only show that \(\int \psi = 1\). Consider
\begin{equation}\begin{aligned}
\left | 1 - \int \psi \right | &= \left | \int (\psi_n - \psi) \right |\\
&\leq \int |\psi_n - \psi|\\
&= \int |\ind_{[-a,a]} (\psi_n - \psi)|\\
&\leq \|\ind_{[-a,a]}\|\cdot\|\psi_n - \psi\|\\
&= 2a\cdot\|\psi_n - \psi\| \to 0,
\end{aligned}\end{equation}
which gives the result.
\end{proof}

Let the unconstrained estimator \(f_n^\alpha\) projected to \(\cC_a\) be denoted
\begin{equation}
\mathring f_n^\alpha = P_{\cC_a} f_n^\alpha.
\end{equation}
The projection operator onto closed convex \(\cC_a\) is non-expansive
(\cite{engl_regularization_1996}, Section 5.4), meaning that for all
\(u,v \in L_2(\RR)\),
\begin{equation}
\|P_{\cC_a}u - P_{\cC_a}v\| \leq \|u - v\|.
\end{equation}
This suggests that \(\mathring f_n^\alpha\) may inherit all of the
consistency and rate properties from \(f_n^\alpha\). Indeed, if \(f
\in \cC_a\), then it is immediate, since \(P_{\cC_a}f = f\), so that
\begin{equation}
\|\mathring f_n^\alpha - f\| = \|P_{\cC_a}f_n^\alpha - Pf\| \leq \|f_n^\alpha - f\|.
\end{equation}

If \(f \not\in \cC_a\) for any \(a\), we need to do a little more
work, and for that we will need to know the size of \(\|P_{\cC_a}f -
f\|\) in terms of \(a\).

\begin{prop}\label{prop:projf}
Assume \(\EE[|X|] < \infty\) and that \(f(t) = o(1)\) as \(|t| \to \infty\)\footnote{This tail condition may be automatic if \(f \in L_2(\RR)\)?}.
Then for \(a\) large enough,
\begin{equation}
\|P_{\cC_a}f - f\| \leq 2\EE[|X|]/a.
\end{equation}
\end{prop}
\begin{proof}{(Proof of Proposition \ref{prop:projf})}
Let \(T_a = \int \ind_{[-a,a]^c}f\) be the quantity of mass \(f\) puts
outside of \([-a,a]\), and note that
\begin{equation}
T_a = \PP(|X| > a) \leq \EE[|X|]/a
\end{equation}
by Markov's inequality. We introduce an element of \(\cC_a\) which is close to \(f\):
\begin{equation}
\psi_a = \ind_{[-a,a]}(f + T_a/2a).
\end{equation}
Then
\begin{equation}\begin{aligned}
\|\psi_a - f\| &= \|\ind_{[-a,a]}(f + T_a/2a) - \ind_{[-a,a]}f - \ind_{[-a,a]^c}f\|\\
&= \|\ind_{[-a,a]}T_a/2a - \ind_{[-a,a]^c}f\|\\
&\leq \|\ind_{[-a,a]}T_a/2a\| + \|\ind_{[-a,a]^c}f\|\\
&= T_a + \|\ind_{[-a,a]^c}f\|.
\end{aligned}\end{equation}
Now,
\begin{equation}\begin{aligned}
\|\ind_{[-a,a]^c}f\| &= \int \ind_{[-a,a]^c} f^2\\
&\leq \int \ind_{[-a,a]^c} f = T_a\\
\end{aligned}\end{equation}
for \(a\) large enough that \(f(t) < 1\) for all \(|t| > a\).
Thus \(\|P_{\cC_a}f - f\| \leq \|\psi_a - f\| \leq 2T_a \leq 2\EE[|X|]/a\), as needed.
\end{proof}

With this in hand, we can say that our constrained estimator will be
as good (in an asymptotic sense) as the unconstrained estimator, as
long as we let \(a\) grow fast enough that the first term dominates:
\begin{lemma}\label{lem:asgood}
Assume \(\EE[|X|] < \infty\) and that \(f(t) = o(1)\) as \(|t| \to \infty\). Then
\begin{equation}
\|\mathring f_n^\alpha - f\| \leq \|f_n^\alpha - f\| + C/a.
\end{equation}
\end{lemma}
\begin{proof}{Proof of \ref{lem:asgood}}
Add and subtract \(P_{\cC_a}f\):
\begin{equation}\begin{aligned}
\|\mathring f_n^\alpha - f\| &= \|P_{\cC_a}f_n^\alpha - P_{\cC_a}f + P_{\cC_a}f - f\|\\
&\leq \|P_{\cC_a}f_n^\alpha - P_{\cC_a}f\| + \|P_{\cC_a}f - f\|\\
&\leq \|f_n^\alpha - f\| + 2\EE[|X|]/a.
\end{aligned}\end{equation}
\end{proof}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../tikhonov"
%%% End:


==> sections/asymptotics_consistency.tex <==
\textcolor{red}{Add pointwise results, which I think have similar proofs.}

It will turn out that the second term in Lemma \ref{lem:upper}
vanishes as \(\alpha \to 0\), but clearly for fixed \(\delta_n^2\),
the first term increases as \(\alpha \to 0\). For consistency,
therefore, we need \(\alpha\) to decrease, but slowly enough to
guarantee that the first term vanishes.

\begin{theorem}{(Global consistency)}\label{theorem:consistency}
 Assume that \(\alpha_n\) is chosen so that \(\delta_n^2/\alpha_n \to
 0\) and \(\alpha_n \to 0\). Then
\[
\lim_{n \to \infty} \mathbb{E} \| f^{\alpha_n}_n - f\|^2 = 0.
\]
\end{theorem}

\input{proofs/theorem:consistency}

Note that Theorem \ref{theorem:consistency} holds under weak
conditions. We assumed that \(g\) is known, but the only property we
need is that it have a.e. non-vanishing Fourier transform, and the
only assumption on the target density \(f\) is that \(f \in
L_2(\mathbb{R})\). All that is required is a consistent estimator \(h_n\) of
\(h\).


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../JASA-template"
%%% End:


==> sections/asymptotics_constrained.tex <==
We know \emph{a priori} that \(f\) is a probability density function, so we
ought to ensure that our estimate is a probability density function as
well. Consider the set \(\cC = \{v \in L_2(\RR): \int v(t)\,dt = 1, \,
v(t) \geq 0\, \forall t \in \RR\}\); this is the set of
square-integrable probability density functions, and now we can
express this requirement as \(f_n^\alpha \in \cC\). One easy-to-manage
approach is to first solve the unconstrained problem and find an
estimate \(f_n^\alpha \not\in \cC\), and then somehow project this
unconstrained estimate onto \(\cC\).

Define the projection operator \(P_A\) onto a closed, convex set \(A
\subset L_2(\RR)\) by
\begin{equation}
P_Au = \argmin_{v \in A} \|u - v\|.
\end{equation}
In words, \(P_A\) maps \(u\) to the nearest (in \(L_2\)) element of \(A\).

Unfortunately, while \(\cC\) is convex, it is not closed. To see this,
note that the zero function is a limit point of \(\cC\): let \(\psi_n
= \frac1n \ind_{[0,n]}\), and note that \(\|\psi_n - 0\| = \|\psi_n\|
= n^{-\frac12} \to 0\) as \(n \to \infty\). Indeed, any non-negative 
function \(v\) with \(\int v < 1\) is a limit point of \(\cC\). Thus
the infimum may not be attained, and the projection operator \(P_\cC\)
is not well-defined.

Instead, we will need to work with approximations to \(\cC\). Let
\[
\cC_a = \{v \in \cC,\,v(t) = 0\,\,\forall t \not\in[-a,a]\}
\]
be the subset of \(\cC\) of functions with support contained in
\([-a,a]\). 
\begin{prop}\label{prop:cCaclosed}
For fixed \(a\), the set \(\cC_a\) is closed and convex.
\end{prop}
\begin{proof}{(Proof of Proposition \ref{prop:cCaclosed})}
Clearly \(\cC_a\) is convex. To see that it is closed, we must show
that any limit point of \(\cC_a\) is also an element of \(\cC_a\). To
that end, suppose \(\{\psi_n\}\subset \cC_a\) and that there is some
\(\psi \in L_2(\RR)\) with \(\|\psi_n - \psi\| \to 0\). Clearly
\(\psi\) is non-negative and has support contained in \([-a,a]\). We
need only show that \(\int \psi = 1\). Consider
\begin{equation}\begin{aligned}
\left | 1 - \int \psi \right | &= \left | \int (\psi_n - \psi) \right |\\
&\leq \int |\psi_n - \psi|\\
&= \int |\ind_{[-a,a]} (\psi_n - \psi)|\\
&\leq \|\ind_{[-a,a]}\|\cdot\|\psi_n - \psi\|\\
&= 2a\cdot\|\psi_n - \psi\| \to 0,
\end{aligned}\end{equation}
which gives the result.
\end{proof}

Let the unconstrained estimator \(f_n^\alpha\) projected to \(\cC_a\) be denoted
\begin{equation}
\mathring f_n^\alpha = P_{\cC_a} f_n^\alpha.
\end{equation}
The projection operator onto closed convex \(\cC_a\) is non-expansive
(\cite{engl_regularization_1996}, Section 5.4), meaning that for all
\(u,v \in L_2(\RR)\),
\begin{equation}
\|P_{\cC_a}u - P_{\cC_a}v\| \leq \|u - v\|.
\end{equation}
This suggests that \(\mathring f_n^\alpha\) may inherit all of the
consistency and rate properties from \(f_n^\alpha\). Indeed, if \(f
\in \cC_a\), then it is immediate, since \(P_{\cC_a}f = f\), so that
\begin{equation}
\|\mathring f_n^\alpha - f\| = \|P_{\cC_a}f_n^\alpha - Pf\| \leq \|f_n^\alpha - f\|.
\end{equation}

If \(f \not\in \cC_a\) for any \(a\), we need to do a little more
work, and for that we will need to know the size of \(\|P_{\cC_a}f -
f\|\) in terms of \(a\).

\begin{prop}\label{prop:projf}
Assume \(\EE[|X|] < \infty\) and that \(f(t) = o(1)\) as \(|t| \to \infty\)\footnote{This tail condition may be automatic if \(f \in L_2(\RR)\)?}.
Then for \(a\) large enough,
\begin{equation}
\|P_{\cC_a}f - f\| \leq 2\EE[|X|]/a.
\end{equation}
\end{prop}
\begin{proof}{(Proof of Proposition \ref{prop:projf})}
Let \(T_a = \int \ind_{[-a,a]^c}f\) be the quantity of mass \(f\) puts
outside of \([-a,a]\), and note that
\begin{equation}
T_a = \PP(|X| > a) \leq \EE[|X|]/a
\end{equation}
by Markov's inequality. We introduce an element of \(\cC_a\) which is close to \(f\):
\begin{equation}
\psi_a = \ind_{[-a,a]}(f + T_a/2a).
\end{equation}
Then
\begin{equation}\begin{aligned}
\|\psi_a - f\| &= \|\ind_{[-a,a]}(f + T_a/2a) - \ind_{[-a,a]}f - \ind_{[-a,a]^c}f\|\\
&= \|\ind_{[-a,a]}T_a/2a - \ind_{[-a,a]^c}f\|\\
&\leq \|\ind_{[-a,a]}T_a/2a\| + \|\ind_{[-a,a]^c}f\|\\
&= T_a + \|\ind_{[-a,a]^c}f\|.
\end{aligned}\end{equation}
Now,
\begin{equation}\begin{aligned}
\|\ind_{[-a,a]^c}f\| &= \int \ind_{[-a,a]^c} f^2\\
&\leq \int \ind_{[-a,a]^c} f = T_a\\
\end{aligned}\end{equation}
for \(a\) large enough that \(f(t) < 1\) for all \(|t| > a\).
Thus \(\|P_{\cC_a}f - f\| \leq \|\psi_a - f\| \leq 2T_a \leq 2\EE[|X|]/a\), as needed.
\end{proof}

With this in hand, we can say that our constrained estimator will be
as good (in an asymptotic sense) as the unconstrained estimator, as
long as we let \(a\) grow fast enough that the first term dominates:
\begin{lemma}\label{lem:asgood}
Assume \(\EE[|X|] < \infty\) and that \(f(t) = o(1)\) as \(|t| \to \infty\). Then
\begin{equation}
\|\mathring f_n^\alpha - f\| \leq \|f_n^\alpha - f\| + C/a.
\end{equation}
\end{lemma}
\begin{proof}{Proof of \ref{lem:asgood}}
Add and subtract \(P_{\cC_a}f\):
\begin{equation}\begin{aligned}
\|\mathring f_n^\alpha - f\| &= \|P_{\cC_a}f_n^\alpha - P_{\cC_a}f + P_{\cC_a}f - f\|\\
&\leq \|P_{\cC_a}f_n^\alpha - P_{\cC_a}f\| + \|P_{\cC_a}f - f\|\\
&\leq \|f_n^\alpha - f\| + 2\EE[|X|]/a.
\end{aligned}\end{equation}
\end{proof}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../tikhonov"
%%% End:


==> sections/asymptotics_rates.tex <==
In deriving rates of convergence for ill-posed problems, it is assumed
that the solution \(f\) is drawn from a ``source set,'' assuming some
\emph{a priori} degree of smoothness (\cite{engl_regularization_1996},
Section 3.2). In \cite{nair_trade-off_1997} Theorem 5.1 and
\cite{engl_optimal_1985} Theorem 3.5, an abstract version of this
Tikhonov problem is analyzed. It is assumed that the target density
\(f \in \mathcal{D}(L^*L)\) and \(L^*Lf \in \mathcal{R}(K^*K)\). This assumption is
rather extreme. Namely, it says that \(f^{(2m)} = g*g*\psi\) for some
\(\psi \in L_2(\mathbb{R})\); some consequences are that \(f\) has at least
twice plus \(2m\) as many \(L_2\) derivatives as \(g\), and \(\Var(X)
\geq 2\Var(\varepsilon)\). Nevertheless, if one can make this
assumption on \(f\), it is possible to compute rates of convergence
with no further assumptions on \(g\).

\begin{theorem}{(Rates when \(f\) is very smooth)}
\label{theorem:smoothrates}
Suppose \(f\) has four \(L_2(\mathbb{R})\) weak derivatives, and \(f^{(4)} =
g*g*\psi\) for some \(\psi \in L_2(\mathbb{R})\). Then for sufficiently small
\(\alpha_n\),
\[
\mathbb{E}\|f^{\alpha_n}_n - f\|^2 \leq C_1 \delta_n^2/\alpha_n + C_2\alpha_n^2,
\]
and if \(\alpha_n = C_3 \delta^{\frac23}\), then
\[
\mathbb{E} \|f^{\alpha_n}_n - f\|^2 = O(\delta_n^\frac43).
\]
\end{theorem}
\begin{proof}{(Proof of Theorem \ref{theorem:smoothrates})}
Our task is to find the dependence of \(\|f^\alpha - f\|^2\) on
\(\alpha\). Taking Fourier transforms yields \(\omega^4 \tilde
f(\omega) = \tilde g(\omega)^2 \tilde \psi(\omega)\). Then we have
\begin{equation}\begin{aligned}
\|f^\alpha - f\|^2 &= \frac{1}{2\pi}\|\tilde f^\alpha - \tilde f\|^2\\
&= \frac{1}{2\pi} \int_P  \left [ \frac{\alpha_n \omega^{2m}}{\tilde g(\omega)^2 + \alpha_n \omega^{2m}}\right ]^2 |\tilde f(\omega)|^2 \,d\omega,\\
&= \frac{1}{2\pi} \int_P  \left [ \frac{\alpha_n \omega^{2m}}{\tilde g(\omega)^2 + \alpha_n \omega^{2m}}\right ]^2 |\omega^{-2m}\tilde \psi(\omega)/\tilde g(\omega)^2|^2 \,d\omega,\\
&= \frac{\alpha_n^2}{2\pi} \int_P  \left [ \frac{\tilde g(\omega)^2}{\tilde g(\omega)^2 + \alpha_n \omega^{2m}}\right ]^2 |\tilde \psi(\omega)|^2 \,d\omega\\
&\leq \alpha_n^2 \|\psi\|^2,
\end{aligned}\end{equation}
which, combined with Lemma \ref{lem:upper}, gives the bound with \(C_2 = \|\psi\|^2\).

Note that the upper bound is minimized by \(\alpha_n =
(C_1/2C_2)^\frac13 \delta_n^\frac23\). If we set \(\alpha_n = C_3
\delta_n^\frac23\), the upper bound becomes
\begin{equation}\begin{aligned}
\mathbb{E}\|f_n - f\|^2 &\leq C_1 C_3 \delta_n^\frac43 + C_2 C_3 \delta_n^\frac43\\
&\leq \max \{C_1, C_2\} C_3 \delta_n^\frac43,
\end{aligned}\end{equation}
from which it follows that
\begin{equation}
\mathbb{E} \|f_n - f\|^2 = O(\delta_n^\frac43).
\end{equation}
\end{proof}

\begin{cor}\label{cor:smoothrates}
Assume the conditions of Theorem \ref{theorem:smoothrates}, and assume that \(\alpha_n = C\delta_n^\frac23\).\\
If \(h_n\) is a kernel density estimate with optimal choice of bandwidth, then
\begin{equation}
\mathbb{E} \|f^{\alpha_n}_n - f\|^2 = O(n^{-8/15}).
\end{equation}

\noindent If \(h_n\) is a histogram with optimal choice of bin widths, then
\begin{equation}
\mathbb{E} \|f^{\alpha_n}_n - f\|^2 = O(n^{-4/9}).
\end{equation}
\end{cor}

\begin{proof}{(Proof of Corollary \ref{cor:smoothrates})}
If \(h_n\) is a kernel density estimate with optimal bandwidth, then
\(\delta_n^2 = \|h_n - h\|^2 = O(n^{-\frac45})\)
(\cite{wand_kernel_1994}, Section 2.5), and the result follows
immediately. Similarly, if \(h_n\) is a histogram with optimal binwidth, then by the same section,
\(\delta_n^2 = \|h_n - h\| = O(n^{-\frac23})\).
\end{proof}

Theorem \ref{theorem:smoothrates} has a nice interpretation: as long
as \(f\) is ``smooth enough,'' where ``smooth enough'' is a criterion
in terms of \(g\), then \(f_n^\alpha\) can attain the same algebraic
rates, regardless of the particular properties of \(g\). However, from
a practical point of view, the character of the assumption is
epistemically backwards: we must know \(g\) exactly to compute the
estimator, and \(f\) is the unknown that we desire to estimate, while
Theorem \ref{theorem:smoothrates} uses little about \(g\) and uses
strong smoothness properties of \(f\). Rates reflecting a
practicioner's point of view will want to use full knowledge of \(g\),
but make weak assumptions about \(f\). To that end, in Lemma
\ref{lem:systematic_bounds} and Theorem \ref{theorem:rates}, we assume
a particular form for \(g\) -- either Gaussian, Cauchy, or Laplace --
and only that \(\|\omega^k \tilde f(\omega)\|<M\) to develop an upper
bound for \(\|f^\alpha - f\|^2\) and derive rates of convergence for
\(\mathbb{E}\|f_n^\alpha - f\|^2\).

\begin{figure}\label{fig:thm1ii}
\center
\input{tikz_plots/laplace_proof}
\vspace{-0.2cm}
\caption{Approach in proof of Lemma \ref{lem:systematic_bounds}, with \(m = 2, k = 2, \alpha = 1/10\). Thick dashed line is \(|\theta(\omega)|\). Thin solid lines are \(\alpha \omega^{2m-k}(1+\omega^2)^2\) and \(\omega^{-k}\). Thin dotted line is \(4\alpha\omega^{2m-k+2}\). Marked point is upper bound for \(|\theta(\omega)|\).}
\end{figure}

\begin{lemma}\label{lem:systematic_bounds}
  Assume \(C \vcentcolon = \frac{1}{2\pi}\int |\omega^k \tilde f(\omega)|^2\,d\omega < \infty\), with \(1 \leq k \leq 2m\). Then
  \begin{enumerate}[label=(\roman*)]
  \item (Normal errors) If \(g(x) = (2\pi)^{-1} e^{-x^2/2}\), 
    then
    \[
      \|f^\alpha - f\|^2 \leq \frac{C}{m^kW(1/(m\alpha^{1/m}))^k} \sim
      \frac{C}{m^k\log(1/(m\alpha^{1/m}))^k}
    \]
  \item (Cauchy errors) If \(g(x) = \frac{1}{\pi(1+x^2)}\), then
  \[
    \|f^\alpha - f\|^2 \leq \frac{C}{m^{2k}W(m^{-1}\alpha^{-\frac{1}{2m}})^{2k}} \sim
    \frac{C}{m^{2k}\log(m^{-1}\alpha^{-\frac{1}{2m}})^{2k}}
  \]
  \item (Laplace errors) If \(g(x) = \frac{1}{2}e^{-|x|}\), then
  \[
    \|f^\alpha - f\|^2 \leq C\left ( \frac{1}{4\alpha} \right )^{-\frac{k}{m+1}},
  \]
  \end{enumerate}
\end{lemma}
\begin{proof}{(Proof of Theorem \ref{lem:systematic_bounds})}
  We first introduce some notions that will be helpful in all three cases, and then we dive into the particulars. Note that
  \begin{equation}
    \begin{aligned}
      \tilde f^\alpha - \tilde f &= \tilde \varphi_\alpha \tilde h - \tilde f\\
      &= \tilde \varphi_\alpha \tilde g \tilde f - \tilde f\\
      &= (\tilde \varphi_\alpha \tilde g - 1)\tilde f.
    \end{aligned}
  \end{equation}
  Now,
  \begin{equation}
    \begin{aligned}
      \tilde \varphi_\alpha(\omega) \tilde g(\omega) - 1 &= \frac{\tilde g(\omega)^2}{\tilde g(\omega)^2 + \alpha \omega^{2m}} - \frac{\tilde g(\omega)^2 + \alpha \omega^{2m}}{\tilde g(\omega)^2 + \alpha \omega^{2m}}\\
      &= \frac{\alpha \omega^{2m}}{\tilde g(\omega)^2 + \alpha \omega^{2m}},
    \end{aligned}
  \end{equation}
  so if we define
  \begin{equation}
    \theta(\omega) \vcentcolon = \frac{\alpha \omega^{2m-k}}{\tilde g(\omega)^2 + \alpha \omega^{2m}},
  \end{equation}
  then we can bound the systematic error in the following way:
  
  \begin{equation}\begin{aligned}
      \|f^\alpha - f\|^2 &= (2\pi)^{-1} \|\tilde f^\alpha -\tilde f\|^2\\
      &= (2\pi)^{-1} \int \left [ \frac{\alpha \omega^{2m}}{\tilde g(\omega)^2 + \alpha \omega^{2m}} \right ]^2 |\tilde f(\omega)|^2 \,d\omega\\
      &= (2\pi)^{-1} \int |\theta(\omega)|^2 |\omega^k\tilde f(\omega)|^2 \,d\omega\\
      &\leq C \sup_{\omega>0} |\theta(\omega)|^2,
    \end{aligned}\end{equation}
  where we can restrict the domain of the supremum to strictly positive \(\omega\) because \(|\theta(\omega)|^2\) is an even, non-negative function and \(|\theta(0)|^2 = 0\).
  \paragraph{(i) (Normal errors)} For normal errors, we have \(\tilde g(\omega) = e^{\omega^2/2}\), so that
  \begin{equation}
    |\theta(\omega)| = \frac{\alpha \omega^{2m-k}}{e^{-\omega^2} + \alpha \omega^{2m}}
  \end{equation}
  Note that 
\begin{equation}
  \theta(\omega) \leq \alpha \omega^{2m-k}e^{\omega^2}
  \qquad\text{ and }\qquad
  \theta(\omega) \leq \omega^{-k},
\end{equation}
where the upper bounds are increasing and decreasing, respectively, with \(\omega\). Thus
\[
  \sup_{\omega > 0} \theta(\omega) \leq \omega_0^{-k}
\]
with \(\omega_0\) being where the upper bounds intersect, i.e. \(\omega_0>0\) satisfies
\[
  \alpha \omega_0^{2m-k} e^{\omega_0^2} = \omega_0^{-k}.
\]
Taking \(m\)\textsuperscript{th} roots and rearranging, we find
\begin{equation}
(\omega_0^{2}/m) e^{\omega_0^2/m} = 1/(m\alpha^{1/m}),
\end{equation}
so that
\begin{equation}
  \omega_0^2/m = W(1/(m\alpha^{1/m})),
\end{equation}
whence
\begin{equation}
  \omega_0 = \left ( mW(1/(m\alpha^{1/m})) \right )^{\frac12}.
\end{equation}
Thus we have that
\begin{equation}
  \sup_{\omega > 0} |\theta(\omega)| \leq \left ( mW(1/(m\alpha^{1/m})) \right )^{-\frac{k}{2}},
\end{equation}
from which it follows that
\begin{equation}
  \sup_{\omega > 0} |\theta(\omega)|^2 \leq \left ( mW(1/(m\alpha^{1/m})) \right )^{-k},
\end{equation}
giving the result.
\paragraph{(ii) (Cauchy errors)} For Cauchy errors, we have \(\tilde g(\omega) = e^{-|\omega|}\), so
  \begin{equation}
    \theta(\omega) = \frac{\alpha \omega^{2m-k}}{e^{-2|\omega|} + \alpha\omega^{2m}}
  \end{equation}
  and seek \(\sup_{\omega>0}|\theta(\omega)|\). Now we note that for \(\omega > 0\),
  \begin{equation}
    \theta(\omega) \leq \alpha \omega^{2m-k}e^{2\omega}\qquad\text{and}\qquad\theta(\omega) \leq \omega^{-k},
  \end{equation}
  which are increasing and decreasing, respectively, with \(\omega\). Thus \(\sup_{\omega \geq 0} \theta(\omega) \leq \omega_0^{-k}\) with \(\omega_0\) the intersection of the two upper bounds, satisfying \(\alpha \omega_0^{2m-k}e^{2\omega_0} = \omega_0^{-k}\). Re-arranging that equality, we find that
  \begin{equation}
    (\omega_0/m)e^{\omega_0/m} = m^{-1}\alpha^{-\frac{1}{2m}},
  \end{equation}
  so that
  \begin{equation}
    \omega_0 = m W\left(m^{-1} \alpha^{-\frac{1}{2m}}\right).
  \end{equation}
  Thus
  \begin{equation}\begin{aligned}
      \|f^\alpha - f\|^2 &\leq C \sup_\omega \left [ \frac{\alpha \omega^{2m-k}}{e^{-2|\omega|} + \alpha\omega^{2m}} \right ]^2\\
      &\leq  \frac{C}{m^{2k} W(m^{-1}\alpha^{-\frac{1}{2m}})^{2k}}.
  \end{aligned}\end{equation}
\paragraph{(iii) (Laplace errors)} For Laplace errors, we have \(\tilde g(\omega) = (1+\omega^2)^{-1}\), so that
  \begin{equation}
    \theta(\omega) = \frac{\alpha \omega^{2m-k}}{(1+\omega^2)^{-2} + \alpha \omega^{2m}},
  \end{equation}
  i.e.
  \begin{equation}
    \theta(\omega) = \frac{\alpha \omega^{2m-k}(1+\omega^2)^2}{1 + \alpha \omega^{2m}(1+\omega^2)^2},
  \end{equation}
  Since both terms in the denominator are positive, we have that
  \begin{equation}
    \theta(\omega) \leq \alpha \omega^{2m-k}(1+\omega^2)^2\qquad\text{and}\qquad \theta(\omega) \leq \omega^{-k},
  \end{equation}
  where the upper bounds are increasing and decreasing monotonically to \(\infty\) and \(0\), respectively, so that they must intersect exactly once, and the value at the intersection is an upper bound for \(\sup_{\omega} |\theta(\omega)|\). For \(\alpha\) small enough, this intersection occurs at some \(\omega \geq 1\), and for \(\omega \geq 1\), we can simplify one of the upper bounds, so that
  \begin{equation}
    \theta(\omega) \leq \alpha \omega^{2m-k}(1+\omega^2)^2 \leq 4\alpha \omega^{2m-k+4}\qquad\text{and}\qquad \theta(\omega) \leq \omega^{-k}.
  \end{equation}
  Now the intersection of the upper bounds \(4\alpha \omega_0^{2m-k+4} = \omega_0^{-k}\) is found to occur at 
  \begin{equation}
    \omega_0 = \left ( \frac{1}{4\alpha} \right )^{\frac{1}{2m+4}},
  \end{equation}
  so that
  \begin{equation}
    \sup_\omega |\theta(\omega)| \leq \left ( \frac{1}{4\alpha} \right )^{-\frac{k}{2m+4}}
  \end{equation}
  and
  \begin{equation}
    \sup_\omega \theta(\omega)^2 \leq \left ( \frac{1}{4\alpha} \right )^{-\frac{k}{m+2}}
  \end{equation}
  Finally, this yields that
  \begin{equation}
    \|f^\alpha - f\|^2 \leq C\left ( \frac{1}{4\alpha} \right )^{-\frac{k}{m+2}},
  \end{equation}
  as needed.
\end{proof}

\begin{theorem}\label{theorem:rates}
  Under the conditions of Lemma \ref{lem:systematic_bounds},
  \begin{enumerate}[label=(\roman*)]
  \item (Normal errors) If \(g(x) = (2\pi)^{-1} e^{-x^2/2}\) and \(\alpha_n = \delta_n^2 W(\delta_n^{-\frac{2}{k}})^{k}\) then
    \[
      \mathbb{E}\|f_n^\alpha - f\|^2 = O([\log \delta_n^{-1}]^{-k}).
    \]
  \item (Cauchy errors) If \(g(x) = \frac{1}{\pi(1+x^2)}\) and \(\alpha_n = \delta_n^2 W(\delta^{-\frac{1}{k}})^{2k}\), then
  \[
    \mathbb{E}\|f_n^\alpha - f\|^2 = O([\log \delta_n^{-1}]^{-2k}).
  \]
  \item (Laplace errors) If \(g(x) = \frac{1}{2}e^{-|x|}\) and \(\alpha_n = \delta_n^{\frac{2m+4}{k+m+2}}\), then
  \[
    \mathbb{E}\|f_n^\alpha - f\|^2 = O(\delta_n^{\frac{2k}{k+m+2}}).
  \]
  \end{enumerate}
\end{theorem}

\begin{proof}
  blah
  \paragraph{(i) (Normal errors)} 
  From Lemma \ref{lem:upper} and Lemma \ref{lem:systematic_bounds}, we have that
  \begin{equation}\label{eqn:normalupperbound}
    \mathbb{E} \|f_n^{\alpha_n} - f\|^2 \leq C_1\delta_n^2/\alpha_n + \frac{C_2}{m^kW(1/(m\alpha^{1/m}))^k}
  \end{equation}
  We will use \(\alpha_n = \delta_n^2 W(\delta_n^{-\frac{2}{k}})^{k}\), which comes from the heuristic that the two summands in the upper bound ought to decrease at the same rate, i.e. by solving
  \begin{equation}
    \frac{\delta_n^2}{\alpha_n} = \log(\alpha^{-\frac{1}{m}})^{-k},
  \end{equation}
  where the \(\log(\cdot)\) is used in lieu of \(W(\cdot)\) as a
  simplification justified by the fact that \(\log(x) \sim W(x)\) as \(x
  \to \infty\). After solving for \(\alpha_n\), constants are ignored
  with wild abandon to yield a simpler \(\alpha_n\).

  We show that with the above choice of \(\alpha_n\), the bound in
  Equation \ref{eqn:normalupperbound} is asymptotically equivalent to
  \(C[\log \delta_n]^{-k}\). Plugging
  \(\alpha_n\) into the first term, we get
  \begin{equation}\begin{aligned}
      C_1 \delta_n^2/\alpha_n &= C_1 W(\delta_n^{-\frac{2}{k}})^{-k}.
    \end{aligned}\end{equation}
  For the second, we have (equivalences are as \(\alpha_n \to 0\) or \(\delta_n \to 0\))
  \begin{equation}\begin{aligned}
      \frac{C_2}{m^kW(1/(m\alpha^{1/m}))^k}  &\sim C_2m^{-k}\left [\log(m^{-1}\alpha^{-\frac{1}{m}})\right ]^{-k}\\
      &= C_2\left [\log(m^{-m} \alpha_n^{-1})\right ]^{-k}\\
      &= C_2\left [\log(m^{-m} \delta_n^{-2} W(\delta_n^{-\frac{2}{k}})^{-k}) \right ]^{-k}\\
      &= C_2\left [ -m\log(m) - 2\log(\delta_n) - k \log( W(\delta_n^{-\frac{2}{k}}))\right ]^{-k}\\
      &= C_2\left [ -m\log(m) - 2\log(\delta_n) - k \left \{ -\frac{2}{k} \log (\delta_n) - W(\delta_n^{-\frac{2}{k}}) \right \}\right ]^{-k}\\
      &=  \frac{C_2}{\left [-m\log(m)+ k W(\delta_n^{-\frac{2}{k}})  \right ]^k}\\
      &\sim C_3W(\delta_n^{-\frac{2}{k}})^{-k}\\
    \end{aligned}\end{equation}
  The above leads us to
  \begin{equation}\begin{aligned}
      C_1\delta_n^2/\alpha_n + \frac{C_2}{m^kW(1/(m\alpha^{1/m}))^k} &= O(W(\delta_n^{-\frac{2}{k}})^{-k})\\
      &=O(\log(\delta_n^{-\frac{2}{k}})^{-k})\\
      &=O(\log(\delta_n^{-1})^{-k})\\
    \end{aligned}\end{equation}
  giving the result.
  \paragraph{(ii) (Cauchy errors)} We find our \(\alpha_n\) again by the heuristic of solving
  \begin{equation}
    \delta_n^2/\alpha_n = \log(\alpha_n^{-\frac{1}{2m}})^{-2k}.
  \end{equation}
  This yields (again, flagrantly dropping constants wherever they appear) \(\alpha_n = \delta_n^2 W(\delta^{-\frac{1}{k}})^{2k}\).
  From Lemma \ref{lem:upper} and Lemma \ref{lem:systematic_bounds}, we find that
  \begin{equation}\label{eqn:cauchyupperbound}
    \mathbb{E} \|f_n^{\alpha_n} - f\|^2 \leq C_1\delta_n^2/\alpha_n + \frac{C_2}{m^{2k}W(m^{-1}\alpha_n^{-\frac{1}{2m}})^{2k}}
  \end{equation}
  The first term, with our choice of \(\alpha_n\), yields
  \begin{equation}
    C_1 \delta_n^2/\alpha_n = C_1 W(\delta_n^{-\frac{1}{k}})^{-2k}.
  \end{equation}
  The second term is
  \begin{equation}\begin{aligned}
    C_2m^{-2k}W(m^{-1}\alpha^{-\frac{1}{2m}})^{-2k} &\sim C_2m^{-2k}\log(m^{-1}\alpha^{-\frac{1}{2m}})^{-2k}\\
    &= C_2m^{-2k}\log(m^{-1}\delta_n^{-\frac{1}{m}} W(\delta_n^{-\frac{1}{k}})^{-2k})\\
    &= C_2m^{-2k}[\log(m^{-1}) - \frac{1}{m} \log(\delta_n) - \frac{k}{m}\log(W(\delta_n^{-\frac{1}{k}}))]^{-2k}\\
    &= C_2m^{-2k}[\log(m^{-1}) + \frac{k}{m}W(\delta_n^{-\frac{1}{k}})]^{-2k}\\
    &\sim C_3[W(\delta_n^{-\frac{1}{k}})]^{-2k}.
  \end{aligned}\end{equation}
Combining the two terms, we find that
\begin{equation}\begin{aligned}
    \mathbb{E} \|f_n^{\alpha_n} - f\|^2 &= O(W(\delta_n^{-\frac{1}{k}})^{-2k})\\
    &= O(\log(\delta_n^{-\frac{1}{k}})^{-2k})\\
    &= O(\log(\delta_n^{-1})^{-2k})\\
\end{aligned}\end{equation}
  \paragraph{(iii) (Laplace errors)}
  We find our \(\alpha_n\) again by the heuristic of solving
  \begin{equation}
    \delta_n^2/\alpha_n = \alpha_n^{\frac{k}{m+2}},
  \end{equation}
  which yields
  \begin{equation}
    \alpha_n = \delta_n^{\frac{2m+4}{k+m+2}}.
  \end{equation}
  Now Lemma \ref{lem:systematic_bounds} combined with Lemma \ref{lem:upper} yields, for sufficiently small \(\alpha_n\),
  \begin{equation}\begin{aligned}
      \|f_n^\alpha - f\|^2 &\leq C_1 \delta_n^2 \alpha_n^{-1} + C_2\alpha_n^{\frac{k}{m+2}}\\
      &= C_3 \delta_n^{\frac{2k}{k+m+2}}\\
    \end{aligned}\end{equation}
  giving the result.
\end{proof}

\begin{cor}
  [This will be a corollary which chooses \(k = 1\) and particular \(h_n\) and shows the results of Theorem \ref{theorem:rates} in the context of the optimal rates from \cite{zhang_fourier_1990}]
\end{cor}

\begin{ex}
  [This will be a series of examples showing particular examples of \(f\) which satisfy the conditions of Theorem \ref{theorem:rates} but not Theorem \ref{theorem:smoothrates}, or satsify the conditions of both, and the rates attained in those cases. We will see that Theorem \ref{theorem:smoothrates} may demand more derivates if \(g\) has many derivatives, and that either way, Theorem \ref{theorem:smoothrates} demands something else -- a kind of ``width'' requirement expressed through the convolution criterion.]
\end{ex}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../tikhonov"
%%% End:


==> sections/elided_theorems_to_save.tex <==
\begin{prop}{(Normal errors, i.)}\label{prop:normali}
Assume \(g(x) = (2\pi)^{-1} e^{-x^2/2}\), and assume \(\int |\omega^k \tilde f(\omega)|^2\,d\omega < \infty\), with \(1 \leq k \leq 2m\).
Then
\[
\|f^\alpha - f\|^2 \leq \frac{C}{m^kW(1/(m\alpha^{1/m}))^k} \sim \frac{C}{m^k\log(1/(m\alpha^{1/m}))^k}
\]
where \(W\) is the principal branch of the Lambert \(W\) function, and \(C = \|\omega^k\tilde f(\omega)\|^2/2\pi\).
\end{prop}
\begin{proof}{(Proof of Proposition \ref{prop:normali})}
\textcolor{red}{(Refer to relevant summary of facts in Fact \ref{fact:lambertW})}\\
First, note that
\begin{equation}\begin{aligned}
\|f^\alpha - f\|^2 &= (2\pi)^{-1} \|\tilde f^\alpha -\tilde f\|^2\\
&= (2\pi)^{-1} \int \left [ \frac{\alpha \omega^{2m}}{e^{-\omega^2} + \alpha \omega^{2m}} \right ]^2 |\tilde f(\omega)|^2 \,d\omega\\
&= (2\pi)^{-1} \int \left [ \frac{\alpha \omega^{2m-k}}{e^{-\omega^2} + \alpha \omega^{2m}} \right ]^2 |\omega^k\tilde f(\omega)|^2 \,d\omega\\
&\leq C \sup_{\omega} \left [ \frac{\alpha \omega^{2m-k}}{e^{-\omega^2} + \alpha \omega^{2m}} \right ]^2
\end{aligned}\end{equation}
by assumption. Now, we address the value of \(\sup_{\omega} \left [
\frac{\alpha \omega^{2m-k}}{e^{-\omega^2} + \alpha \omega^{2m}} \right
]^2\). Let \(\theta(\omega) = \frac{\alpha
\omega^{2m-k}}{e^{-\omega^2} + \alpha \omega^{2m}}\), and since
\(|\theta(\omega)|\) is even, we will only consider \(\omega > 0\),
and seek \(\sup_{\omega > 0} \theta(\omega).\) To that end, note that
\begin{equation}
  \theta(\omega) \leq \alpha \omega^{2m-k}e^{\omega^2}
  \qquad\text{ and }\qquad
  \theta(\omega) \leq \omega^{-k},
\end{equation}
where the upper bounds are increasing and decreasing, respectively, with \(\omega\). Thus
\[
  \sup_{\omega > 0} \theta(\omega) \leq \omega_0^{-k}
\]
with \(\omega_0\) being where the upper bounds intersect, i.e. \(\omega_0>0\) satisfies
\[
  \alpha \omega_0^{2m-k} e^{\omega_0^2} = \omega_0^{-k}.
\]
Taking \(m\)\textsuperscript{th} roots and rearranging, we find
\begin{equation}
(\omega_0^{2}/m) e^{\omega_0^2/m} = 1/(m\alpha^{1/m}),
\end{equation}
so that
\begin{equation}
  \omega_0^2/m = W(1/(m\alpha^{1/m})),
\end{equation}
whence
\begin{equation}
  \omega_0 = \left ( mW(1/(m\alpha^{1/m})) \right )^{\frac12}.
\end{equation}
Thus we have that
\begin{equation}
  \sup_{\omega > 0} \theta(\omega) \leq \left ( mW(1/(m\alpha^{1/m})) \right )^{-\frac{k}{2}},
\end{equation}
from which it follows that
\begin{equation}
  \sup_{\omega} \left [\frac{\alpha \omega^{2m-k}}{e^{-\omega^2} + \alpha \omega^{2m}} \right]^2 = \sup_{\omega > 0} \theta(\omega)^2 \leq \left ( mW(1/(m\alpha^{1/m})) \right )^{-k},
\end{equation}
giving the result.
\end{proof}

\begin{theorem}{(Normal errors, ii.)}\label{theorem:normalii}
Assume the conditions of Proposition \ref{prop:normali}. There
is a choice of \(\alpha_n \to 0\) for which
\[
\EE\|f_n^\alpha - f\|^2 = O([\log \delta_n^{-1}]^{-k}).
\]
\end{theorem}
\begin{proof}{(Proof of Theorem \ref{theorem:normalii})}
From Lemma \ref{lem:upper} and Proposition \ref{prop:normali}, we have that
\begin{equation}\label{eqn:normalupperbound}
\EE \|f_n^{\alpha_n} - f\|^2 \leq C_1\delta_n^2/\alpha_n + \frac{C_2}{m^kW(1/(m\alpha^{1/m}))^k}
\end{equation}
We will use \(\alpha_n = \delta_n^2 W(\delta_n^{-\frac{2}{k}})^{k}\), which comes from the heuristic that the two summands in the upper bound ought to decrease at the same rate, i.e. by solving
\begin{equation}
  \frac{\delta_n^2}{\alpha_n} = \log(\alpha^{-\frac{1}{m}})^{-k},
\end{equation}
where the \(\log(\cdot)\) is used in lieu of \(W(\cdot)\) as a
simplification justified by the fact that \(\log(x) \sim W(x)\) as \(x
\to \infty\). After solving for \(\alpha_n\), constants are ignored
with wild abandon to yield a simpler \(\alpha_n\).

We show that with the above choice of \(\alpha_n\), the bound in
Equation \ref{eqn:normalupperbound} is asymptotically equivalent to
\(C[\log \delta_n]^{-k}\). Plugging
\(\alpha_n\) into the first term, we get
\begin{equation}\begin{aligned}
C_1 \delta_n^2/\alpha_n &= C_1 W(\delta_n^{-\frac{2}{k}})^{-k}.
\end{aligned}\end{equation}
For the second, we have (equivalences are as \(\alpha_n \to 0\) or \(\delta_n \to 0\))
\begin{equation}\begin{aligned}
\frac{C_2}{m^kW(1/(m\alpha^{1/m}))^k}  &\sim C_2m^{-k}\left [\log(m^{-1}\alpha^{-\frac{1}{m}})\right ]^{-k}\\
&= C_2\left [\log(m^{-m} \alpha_n^{-1})\right ]^{-k}\\
&= C_2\left [\log(m^{-m} \delta_n^{-2} W(\delta_n^{-\frac{2}{k}})^{-k}) \right ]^{-k}\\
&= C_2\left [ -m\log(m) - 2\log(\delta_n) - k \log( W(\delta_n^{-\frac{2}{k}}))\right ]^{-k}\\
&= C_2\left [ -m\log(m) - 2\log(\delta_n) - k \left \{ -\frac{2}{k} \log (\delta_n) - W(\delta_n^{-\frac{2}{k}}) \right \}\right ]^{-k}\\
&=  \frac{C_2}{\left [-m\log(m)+ k W(\delta_n^{-\frac{2}{k}})  \right ]^k}\\
&\sim C_3W(\delta_n^{-\frac{2}{k}})^{-k}\\
\end{aligned}\end{equation}
The above leads us to
\begin{equation}\begin{aligned}
    C_1\delta_n^2/\alpha_n + \frac{C_2}{m^kW(1/(m\alpha^{1/m}))^k} &= O(W(\delta_n^{-\frac{2}{k}})^{-k})\\
    &=O(\log(\delta_n^{-\frac{2}{k}})^{-k})\\
    &=O(\log(\delta_n^{-1})^{-k})\\
\end{aligned}\end{equation}
giving the result.
\end{proof}

\begin{prop}{(Cauchy errors, i.)}\label{prop:cauchyi}
Assume \(g(x) = \frac{1}{\pi(1+x^2)}\), and assume \(\int |\omega^k \tilde f(\omega)|^2\,d\omega < \infty\), with \(1 \leq k \leq 2m\).
Then
\[
\|f^\alpha - f\|^2 \leq \frac{C}{m^{2k}W(m^{-1}\alpha^{-\frac{1}{2m}})^{2k}} \sim \frac{C}{m^{2k}\log(m^{-1}\alpha^{-\frac{1}{2m}})^{2k}}
\]
where \(W\) is the principal branch of the Lambert \(W\) function, and \(C = \|\omega^k\tilde f(\omega)\|^2/2\pi\).
\end{prop}
\begin{proof}{(Proof of Proposition \ref{prop:cauchyi})}
  We proceed as in the proof of Proposition \ref{prop:normali}, except that since \(\tilde g(\omega) = e^{-|\omega|}\), we now set
  \begin{equation}
    \theta(\omega) = \frac{\alpha \omega^{2m-k}}{e^{-2|\omega|} + \alpha\omega^{2m}}
  \end{equation}
  and seek \(\sup_{\omega>0}|\theta(\omega)|\). Now we note that for \(\omega > 0\),
  \begin{equation}
    \theta(\omega) \leq \alpha \omega^{2m-k}e^{2\omega}\qquad\text{and}\qquad\theta(\omega) \leq \omega^{-k},
  \end{equation}
  which are increasing and decreasing, respectively, with \(\omega\). Thus \(\sup_{\omega \geq 0} \theta(\omega) \leq \omega_0^{-k}\) with \(\omega_0\) the intersection of the two upper bounds, satisfying \(\alpha \omega_0^{2m-k}e^{2\omega_0} = \omega_0^{-k}\). Re-arranging that equality, we find that
  \begin{equation}
    (\omega_0/m)e^{\omega_0/m} = m^{-1}\alpha^{-\frac{1}{2m}},
  \end{equation}
  so that
  \begin{equation}
    \omega_0 = m W\left(m^{-1} \alpha^{-\frac{1}{2m}}\right).
  \end{equation}
  Thus
  \begin{equation}\begin{aligned}
      \|f^\alpha - f\|^2 &\leq C \sup_\omega \left [ \frac{\alpha \omega^{2m-k}}{e^{-2|\omega|} + \alpha\omega^{2m}} \right ]^2\\
      &\leq  \frac{C}{m^{2k} W(m^{-1}\alpha^{-\frac{1}{2m}})^{2k}}.
  \end{aligned}\end{equation}
\end{proof}

\begin{theorem}{(Cauchy errors, ii.)}\label{theorem:cauchyii}
Assume the conditions of Proposition \ref{prop:cauchyi}. There
is a choice of \(\alpha_n \to 0\) for which
\[
\EE\|f_n^\alpha - f\|^2 = O([\log \delta_n^{-1}]^{-2k}).
\]
\end{theorem}
\begin{proof}{(Proof of Theorem \ref{theorem:cauchyii})}
  We find our \(\alpha_n\) again by the heuristic of solving
  \begin{equation}
    \delta_n^2/\alpha_n = \log(\alpha_n^{-\frac{1}{2m}})^{-2k}.
  \end{equation}
  This yields (again, flagrantly dropping constants wherever they appear) \(\alpha_n = \delta_n^2 W(\delta^{-\frac{1}{k}})^{2k}\).
  From Lemma \ref{lem:upper} and Proposition \ref{prop:cauchyi}, we find that
  \begin{equation}\label{eqn:cauchyupperbound}
    \EE \|f_n^{\alpha_n} - f\|^2 \leq C_1\delta_n^2/\alpha_n + \frac{C_2}{m^{2k}W(m^{-1}\alpha_n^{-\frac{1}{2m}})^{2k}}
  \end{equation}
  The first term, with our choice of \(\alpha_n\), yields
  \begin{equation}
    C_1 \delta_n^2/\alpha_n = C_1 W(\delta_n^{-\frac{1}{k}})^{-2k}.
  \end{equation}
  The second term is
  \begin{equation}\begin{aligned}
    C_2m^{-2k}W(m^{-1}\alpha^{-\frac{1}{2m}})^{-2k} &\sim C_2m^{-2k}\log(m^{-1}\alpha^{-\frac{1}{2m}})^{-2k}\\
    &= C_2m^{-2k}\log(m^{-1}\delta_n^{-\frac{1}{m}} W(\delta_n^{-\frac{1}{k}})^{-2k})\\
    &= C_2m^{-2k}[\log(m^{-1}) - \frac{1}{m} \log(\delta_n) - \frac{k}{m}\log(W(\delta_n^{-\frac{1}{k}}))]^{-2k}\\
    &= C_2m^{-2k}[\log(m^{-1}) + \frac{k}{m}W(\delta_n^{-\frac{1}{k}})]^{-2k}\\
    &\sim C_3[W(\delta_n^{-\frac{1}{k}})]^{-2k}.
  \end{aligned}\end{equation}
Combining the two terms, we find that
\begin{equation}\begin{aligned}
    \EE \|f_n^{\alpha_n} - f\|^2 &= O(W(\delta_n^{-\frac{1}{k}})^{-2k})\\
    &= O(\log(\delta_n^{-\frac{1}{k}})^{-2k})\\
    &= O(\log(\delta_n^{-1})^{-2k})\\
\end{aligned}\end{equation}
\end{proof}

\begin{prop}{(Laplace errors, i.)}\label{prop:laplacei}
Assume \(g(x) = \frac{1}{2}e^{-|x|}\), and assume \(\int |\omega^k \tilde f(\omega)|^2\,d\omega < \infty\), with \(1 \leq k \leq 2m\).
Then
\[
    \|f^\alpha - f\|^2 \leq C\left ( \frac{1}{2\alpha} \right )^{-\frac{k}{m+1}},
\]
where \(C = \|\omega^k\tilde f(\omega)\|^2/2\pi\).
\end{prop}
\begin{proof}
  We proceed as in the proofs of Propositions \ref{prop:normali} and \ref{prop:cauchyi}, with \(\tilde g(\omega) = (1+\omega^2)^{-1}\), so that
  \begin{equation}
    \theta(\omega) = \frac{\alpha \omega^{2m-k}(1+\omega^2)}{1 + \alpha \omega^{2m}(1+\omega^2)}.
  \end{equation}
  Since \(|\theta(\omega)|\) is symmetric, we may restrict attention to \(\omega > 0\). Since both terms in the denominator are positive, we have that
  \begin{equation}
    \theta(\omega) \leq \alpha \omega^{2m-k}(1+\omega^2)\qquad\text{and}\qquad \theta(\omega) \leq \omega^{-k},
  \end{equation}
  where the upper bounds are increasing and decreasing monotonically to \(\infty\) and \(0\), respectively, so that they must intersect exactly once, and the value at the intersection is an upper bound for \(\sup_{\omega} |\theta(\omega)|\). For \(\alpha\) small enough, this intersection occurs at some \(\omega \geq 1\), and for \(\omega \geq 1\), we can simplify one of the upper bounds, so that
  \begin{equation}
    \theta(\omega) \leq \alpha \omega^{2m-k}(1+\omega^2) \leq 4\alpha \omega^{2m-k+2}\qquad\text{and}\qquad \theta(\omega) \leq \omega^{-k}.
  \end{equation}
  Now the intersection of the upper bounds \(4\alpha \omega_0^{2m-k+2} = \omega_0^{-k}\) is found to occur at 
  \begin{equation}
    \omega_0 = \left ( \frac{1}{4\alpha} \right )^{\frac{1}{2m+2}},
  \end{equation}
  so that
  \begin{equation}
    \sup_\omega |\theta(\omega)| \leq \left ( \frac{1}{4\alpha} \right )^{-\frac{k}{2m+2}}
  \end{equation}
  and
  \begin{equation}
    \sup_\omega \theta(\omega)^2 \leq \left ( \frac{1}{4\alpha} \right )^{-\frac{k}{m+1}}
  \end{equation}
  Finally, this yields that
  \begin{equation}
    \|f^\alpha - f\|^2 \leq C\left ( \frac{1}{4\alpha} \right )^{-\frac{k}{m+1}},
  \end{equation}
  as needed.
\end{proof}
\begin{theorem}{(Laplace errors, ii.)}\label{theorem:laplaceii}
Assume the conditions of Proposition \ref{prop:laplacei}. There
is a choice of \(\alpha_n \to 0\) for which
\[
\EE\|f_n^\alpha - f\|^2 = O(\delta_n^{\frac{2k}{k+m+1}}).
\]
\end{theorem}
\begin{proof}
  We find our \(\alpha_n\) again by the heuristic of solving
  \begin{equation}
    \delta_n^2/\alpha_n = \alpha_n^{\frac{k}{m+1}},
  \end{equation}
  which yields
  \begin{equation}
    \alpha_n = \delta_n^{\frac{2m+2}{k+m+1}}.
  \end{equation}
  Now Proposition \ref{prop:laplacei} combined with Lemma \ref{lem:upper} yields, for sufficiently small \(\alpha_n\),
  \begin{equation}\begin{aligned}
    \|f_n^\alpha - f\|^2 &\leq C_1 \delta_n \alpha_n^{-1} + C_2\alpha_n^{\frac{k}{m+1}}\\
    &= C_3 \delta_n^{\frac{2k}{k+m+1}},
  \end{aligned}\end{equation}
giving the result.
\end{proof}


==> sections/illposed.tex <==
\label{sec:illposed}

Deconvolving a density estimate is a typical ``ill-posed'' problem.
We will see that ill-posedness means a naive solution to the
deconvolution problem must fail to be consistent, and any consistent
deconvolution estimator must have some aspect of regularization.
 A problem is said to be well-posed if \cite[Chapter 2]{engl_regularization_1996},

\begin{enumerate}
 \item For all admissible data, a solution exists,
 \item For all admissible data, the solution is unique, and
 \item The solution depends continuously on the data,
\end{enumerate}
and ill-posed otherwise.  Consider the operator \(T:L_2(\mathbb{R}) \to
L_2(\mathbb{R})\) which convolves a function with \(g\), i.e. \(v \mapsto
g*v\). Since \(h = g*f\), The function \(f\) clearly solves the
following operator equation:
\begin{equation}\label{eqn:exactopeq}
Tv = h.
\end{equation}
The ``obvious'' solution is to compute the inverse of \(T\), but this has 

In our case, \(h = g*f\) and \(f \in L_2(\mathbb{R})\), so we might think:
``take the inverse of \(K\),'' and be done with it. Indeed, this gives a
well-posed problem, but only if ``the data'' (i.e. the right-hand side
of Equation \eqref{eqn:exactopeq}) is taken from the singleton set
\(\{h\}\). But this isn't the problem we truly want to
solve. Instead, we want to solve
\begin{equation}\label{eqn:approxopeq}
Kv = h_n
\end{equation}
for some estimate \(h_n\) of \(h\). Now, ``the data'' refers to the
possible \(h_n\) that we may be using in this approximate problem.
This problem violates the first condition if we allow \(h_n \not \in
\mathcal{R}(K)\) -- say, a histogram estimate -- but we can overcome
this by adjusting what we mean by ``solution,'' and admitting the
least-squares solution \(f_n\) minimizing \(\|Kv - h_n\|\) in \(v\).

However, the third condition takes more work to overcome. The operator
\(K\) is injective (Fact \ref{fact:injective}), so it is invertible
from its range. However, the range \(\mathcal{R}(K)\) is not closed
(Fact \ref{fact:notclosed}). By Proposition 2.4 of
\cite{engl_regularization_1996}, the Moore-Penrose inverse \(K^\dag\),
which extends the inverse of \(K\) from its range, is not
continuous. This can be seen vividly by taking a particular sequence:
the \(\psi_n = n\mathds{1}_{[0,\frac{1}{n}]}\) given in the proof of Fact
\ref{fact:notclosed} have the property that \(\|\psi_{n+1} - \psi_n\|
= 1\), so that we can have \(\|K(\psi_{n+1} - \psi_n)\| \to 0\), while
\(\|K^\dag K(\psi_{n+1}-\psi_n)\| = \|\psi_{n+1} - \psi_n\| =
1\). Thus, even if we could compute the Moore-Penrose inverse of \(K\)
(or indeed any other operator that extends the inverse of \(K\) from
its range), it would be sensitive to small perturbations in the RHS of
Equation \eqref{eqn:approxopeq}, which are inevitable, since \(h_n\) will
be estimated from the data.

The method of Tikhonov regularization approximates the least-squares
solution to Equation \eqref{eqn:approxopeq} by a family of
well-behaved (i.e. continuous) approximate solution operators indexed
by a parameter which governs a trade-off between how stable the
approximate problem is vs. how closely it approximates the ill-posed
problem of interest. That is, as \(\alpha \to 0\), \(f_n^\alpha \to
K^\dag h_n\), but for each \(\alpha\), the map \(h_n \mapsto
f_n^\alpha\) is continuous in \(h_n\).


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper"
%%% End:


==> sections/introduction.tex <==
%\textcolor{red}{Briefly describe the problem in mathy language}\\
Suppose a real-valued random variable of interest \(X\)
has pdf \(f\), and it is desired to estimate \(f\). However, one
instead observes independent copies of \(X+\varepsilon\), a surrogate
of \(X\) which has been contaminated with independent errors
\(\varepsilon\). Suppose further that \(\varepsilon\) has known pdf
\(g\).

%\textcolor{red}{Give application examples}\\
\cite{yang_bias-corrected_2021} [nested simulations]\\
\cite{mendelsohn_deconvolution_1982} [flow microfluorometry for
measuring DNA content of cells]

%\textcolor{red}{Describe previous work on deconvolution}\\
\cite{fan_optimal_1991}\\
\cite{staudenmayer_density_2008}\\
\cite{carroll_optimal_1988}\\
\cite{stefanski_rates_1990}\\
\cite{stefanski_deconvoluting_1990}\\
\cite{zhang_fourier_1990}\\

%\textcolor{red}{Describe the approach taken here, how it differs, and the outline of the paper}\\

The approach that we take here is to minimize the \(L_2(\mathbb{R})\) norm of
the error in reconstructing the density estimate \(h_n\) of \(h\), but
penalize the norm of a measure of smoothness applied to the solution,
in our case the \(m\textsuperscript{th}\) derivative. We do this by
means of minimizing a ``Tikhonov functional,'' given by

\begin{equation}\label{eqn:tikhonov}
G^\alpha_n(v) = \|g*v - h_n\|^2 + \alpha\|v^{(m)}\|^2,\qquad\qquad v \in \mathcal{D}(L)
\end{equation}
This approach balances fidelity to the data through the first term
with stability of the estimation procedure through the second term.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../JASA-template"
%%% End:


==> sections/representation.tex <==

[BLAH BLAH DESCRIPTION OF TIKHONOV REGULARIZATION]

Our estimator will measure the smoothness or regularity of a possible
estimate by the magnitude of its square-integrated \(m\)th derivative,
so the estimate must be chosen from among those functions for which
this quantity is finite. To that end, let \(H^m(\mathbb{R}) = \{v \in
L_2(\mathbb{R}) : v^{k} \in L_2(\mathbb{R})\text{ for }0 \leq k \leq
m\}\) denote the Sobolev space of square-integrable functions with
square-integrable weak derivatives up to order \(m\).

\begin{defn}
  The \emph{Tikhonov functional} with data \(u\in L_2(\mathbb{R})\) and penalty parameter \(\alpha>0\) is a function \(G(\,\cdot\,;u,\alpha): H^m(\mathbb{R}) \to \mathbb{R}\) defined by
  \begin{equation}
    G(v;u,\alpha) = \|g*v - u\|^2 + \alpha \|v^{(m)}\|^2.
  \end{equation}
\end{defn}

\
\begin{defn}
  Let \(h_n\) be a density estimate of \(h\) from the sample \(Y_1, \dots, Y_n\), and let \(\alpha > 0\). The the Tikhonov regularized density estimate of \(f\) is defined variationally by
  \begin{equation}\begin{aligned}
      f_n^\alpha &= \argmin_{v \in H^m(\mathbb{R})}\, G(v;h_n,\alpha) \\
      &= \argmin_{v \in H^m(\mathbb{R})}\,\|g*v - h_n\|^2 + \alpha \|v^{(m)}\|^2.
  \end{aligned}\end{equation}
\end{defn}

In this section, in Theorem \ref{theorem:representing}, we present
an explicit representation for the minimizer \(f^\alpha_n\) of the
Tikhonov functional in Equation \eqref{eqn:tikhonov}, both in terms of
\(h_n\) and its Fourier transform; if a kernel density estimator is
used for \(h_n\), we will see that \(f^\alpha_n\) can be computed as a
kind of kernel density estimate as well, though this is not the
approach we take in the sequel. The Fourier representation will make
clear the manner in which the Tikhonov regularization approximates the
ill-posed inverse problem.

In approaching the deconvolution problem, a reasonable first approach
might be through an appeal to the Fourier transform and associated
Convolution Theorem. The Convolution Theorem says that Fourier
transform reduces convolution to a multiplication operator: \(h = g*f
\Rightarrow \tilde h = \tilde g \tilde f\), so a naive approach might
be to take \(\tilde f_n = \tilde h_n/\tilde g\). Without further
restrictions on admissible \(h_n\), this cannot work, for reasons
related to the arguments of Section \ref{sec:illposed}. First, if
\(h_n \not \in \mathcal{R}(K)\), it is possible that \(\tilde h_n/\tilde g\)
not yield the Fourier transform of an integrable function; see Example
\ref{ex:histogramdecon}. Second, even if \(h_n\) is chosen from
\(\mathcal{R}(K)\), the argument of Section \ref{sec:illposed} demonstrates
that this process cannot be continuous in \(h_n\) if \(h_n\) is
allowed to range across all of \(L_2(\mathbb{R})\) or even \(\mathcal{R}(K)\).

\begin{ex}\label{ex:histogramdecon}
%\textcolor{red}{Add computations for histogram deconvolution by naive approach}
For example, if \(h_n\) is a histogram and \(g\) a Gaussian density,
then \(|\tilde h_n(\omega)/\tilde g(\omega)| \to \infty\) as
\(|\omega| \to \infty\), and therefore \(\mathcal{F}^{-1}[\tilde h_n/\tilde
g]\) is not integrable (cf. Fact \ref{fact:gtwiddle})
\end{ex}

However, this naive approach of dividing \(\tilde h_n\) by \(\tilde
g\) is not altogether ill-conceived. In fact, the minimizer of
Equation \eqref{eqn:tikhonov} can be seen as a well-behaved
approximation to this approach. To see this, we need an expression for
the Fourier transform of \(f_n^\alpha\); in Theorem
\ref{theorem:representing}(i), we will see that it is \(\tilde
f_n^\alpha(\omega) = \frac{\tilde g(\omega)}{\tilde g(\omega)^2 +
\alpha \omega^{2m}}\tilde h_n(\omega) = \tilde \varphi_\alpha(\omega)
\tilde h_n(\omega)\).

\begin{figure}
\center
\input{tikz_plots/approxinv}
\caption{For \(\tilde g\) corresponding to \(\N(0,1)\). Thick line is \(1/\tilde g\), while dashed lines are the multiplier \(\tilde \varphi_\alpha\) in Theorem \ref{theorem:representing}(i) for \(\alpha = 1, 10^{-2}, 10^{-4}\).}
\label{fig:approxinv}
\end{figure}

Inspection of the multiplier \(\tilde \varphi_\alpha(\omega)\) shows
that it may be thought of as an approximation of division by \(\tilde
g\), since in a region around \(\omega = 0\), \(\alpha \omega^{2m}
\approx 0\). However, as \(|\omega| \to \infty\), the \(\alpha
\omega^{2m}\) term dominates the expression, and the multiplier
approaches zero, damping high-frequency components in the
estimate. Figure \ref{fig:approxinv} offers a visualization of this
approximation.

The expression in Theorem \ref{theorem:representing}(i) will also
allow us in Lemma \ref{lem:upper} to upper-bound the error in our
estimate of \(f\) by an expression involving two terms: one involving
the error in our estimate of \(h\), and the other involving the
systematic error that the regularization introduces. We will see in
Theorem \ref{theorem:consistency} that these terms must be balanced to
ensure consistency.

%\textcolor{red}{Is \(\varphi_\alpha\) related to a Green's function??? What is a Green's function???}
\begin{theorem}{(Representing the solution)}
\label{theorem:representing}
Let
\begin{equation}
f^\alpha_n = \argmin_{v \in \mathcal{D}(L)} \|g*v - h_n\|^2 + \alpha \|v^{(m)}\|^2
\end{equation}
and
\begin{equation}\label{eqn:varphi}
  \tilde \varphi_\alpha(\omega) = \frac{\tilde g(\omega)}{\tilde g(\omega)^2 + \alpha \omega^{2m}}.
\end{equation}
For \(m \geq 2\), let 
\begin{equation}
  \varphi_\alpha(x) = \frac{1}{2\pi} \int e^{i\omega x} \tilde \varphi_\alpha(\omega)\,d\omega.
\end{equation}

Then,
\begin{enumerate}[label=(\roman*)]
\item \(\tilde f^\alpha_n(\omega) = \tilde \varphi_\alpha(\omega) \tilde h_n(\omega)\)
\item \(f^\alpha_n(x) = \varphi_\alpha * h_n(x)\) if \(m \geq 2\).
\item If \(h_n\) is a kernel density estimate with bandwidth \(\nu\) and \(m \geq 2\), then there is another kernel \(K_{\alpha,\nu}\) for which
\[f^\alpha_n(x) = \frac{1}{n} \sum_{i=1}^n K_{\alpha,\nu}(x - Y_i).\]
\end{enumerate}
Furthermore,
\begin{enumerate}[label=(\roman*)]\setcounter{enumi}{3}
\item \(\sup_\omega |\tilde \varphi_\alpha(\omega)| \leq C\alpha^{-\frac12}\) for some \(C > 0\) depending only on \(g\), as long as \(\alpha < 1\), and if \(m \geq 2\), we have \(\int |\tilde \varphi_\alpha| \leq C'\alpha^{-\frac12}\) as well, for some \(C' > 0\).
\item If \(\varphi_\alpha \in L_1(\mathbb{R})\), then \(\int \varphi_\alpha(x)\,dx = 1\), so that \(\int f_n^\alpha(x)\,dx = 1\).
\end{enumerate}
\end{theorem}

\begin{remark}
Note that \(\tilde \varphi_\alpha(\omega)\) is even and purely real, since the error density \(g\) is an even function.
\end{remark}

\begin{remark}
Theorem \ref{theorem:representing}(iv) equivalently says that the
operator norm \(\|(T^*T + \alpha L^*L)^{-1}T^*\| \leq
C\alpha^{-\frac12}\) with our particular choices of \(T\) and \(L\),
showing that the solution operator for each approximate problem
(i.e. each \(\alpha\)) is continuous.
\end{remark}

\input{proofs/theorem:representing}

\begin{figure}\label{fig:prop1}\center
\input{tikz_plots/prop1}
\caption{For \(\tilde g\) corresponding to \(\unif[-1,1]\). Solid lines are \(\sqrt{\alpha} |\tilde \varphi_\alpha(\omega)|\) from Theorem \ref{theorem:representing}(iv) with \(\alpha = 1, 0.1, 0.01\). Dotted line is \(\frac12 \omega^{-2}\). Dashed lines are \(\alpha^{\frac12}/\tilde g(\omega)\).}
\end{figure}

%\textcolor{red}{Add expressions for bias and variance at a point.}



\begin{figure}\label{fig:thm1ii}
\center
\input{tikz_plots/thm1ii.tex}
\vspace{-0.2cm}
\caption{Plots of \(\varphi_\alpha(x)\) from Theorem \ref{theorem:representing}. Rows correspond to normal, Laplace, and uniform errors from top to bottom, all with variance \(\sigma^2 = 1/10\). Columns are \(\alpha = 10^{-4}, 10^{-8}, 10^{-12}\) from left to right.}
\end{figure}

As mentioned at the end of Section \ref{sec:illposed}, the
Tikhonov-regularized solution \(f_n^\alpha\) solves an approximation
to the least-squares problem \(\argmin_v \|Kv - h_n\|\). For a fixed
\(\alpha\), it is useful to think of \(f_n^\alpha\) as an estimate of
a smoothed version of \(f\), which we call \(f^\alpha\) (Equation
\eqref{eqn:falpha}) rather than an estimate of \(f\), and think of the
error in \(f_n^\alpha\) as having two components: 1) how well we have
estimated \(f^\alpha\), and 2) how close \(f^\alpha\) is to
\(f\). That is, we write
\begin{equation}
  f_n^\alpha - f = (f_n^\alpha - f^\alpha) + (f^\alpha - f).
\end{equation}
This notion, along with Theorem \ref{theorem:representing}(i,iv),
gives an upper bound for \(\mathbb{E}\|f_n^\alpha - f\|^2\) in terms of
\(\alpha\), \(f\), and \(\delta_n^2 = \mathbb{E}\|h_n - h\|^2\).
\begin{lemma}
\label{lem:upper}
For \(\alpha\) sufficiently small, we have the upper bound
\[
\mathbb{E} \|f_n^\alpha - f\|^2 \leq C\delta_n^2/\alpha + 2\|f^\alpha - f\|^2.
\]
\end{lemma}

\input{proofs/lem:upper}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../JASA-template"
%%% End:


==> sections/setting.tex <==
In the following, \(f \in L_1(\mathbb{R}) \cap L_2(\mathbb{R})\) will be a
probability density function, representing the density which we desire
to estimate. Our observations are contaminated by measurement error
with pdf \(g \in L_1(\mathbb{R})\). We assume throughout that \(g\) is an
even function and that its Fourier transform is almost-everywhere
non-vanishing. If \(X\) has pdf \(f\), and \(\varepsilon\) has pdf
\(g\), then if \(X\) and \(\varepsilon\) are independent, \(Y =
X+\varepsilon\) has pdf \(h = g*f\). Note that \(h \in L_1(\mathbb{R}) \cap
L_2(\mathbb{R})\). We assume that we have a sample \(\{Y_i\}_{i=1}^n\) with
pdf \(h\), i.e., we have observed \(n\) independent,
error-contaminated copies of \(X\). From these, we wish to estimate
\(f\).

In the following, density estimates will be denoted with a subscript
``\(n\),'' so that \(h_n\) represents a density estimate of \(h\) (our
estimates forego ``hats'' to avoid clutter when writing Fourier
transforms). The Tikhonov penalty parameter will be denoted by
\(\alpha\), and a Tikhonov density estimate bears both subscript
``\(n\)'' and superscript ``\(\alpha\),'' i.e. \(f_n^\alpha\) is the
minimizer of \(G^\alpha_n\) in Equation \eqref{eqn:tikhonov}.
Finally, we will refer to the expected error in our density estimate
of \(h\) by \(\delta_n^2 = \mathbb{E} \|h_n - h\|^2\).

``Placeholder'' variables representing functions of \(L_2(\mathbb{R})\) will
typically be denoted by \(u\) or \(v\), and particular but transient
functions and sequences of functions will typically be denoted by
\(\psi\) or \(\psi_n\); that is, each time a sequence \(\psi_n\) is
introduced, it represents a different sequence than the previous
\(\psi_n\).

Fourier transforms will be denoted with a ``twiddle,'' so that the
Fourier transform of \(f\) is denoted \(\tilde f\). The Fourier
convention we use is \(\tilde f(\omega) = \int e^{-i\omega x}
f(x)\,d\omega\). For reference (perhaps mostly to help you keep track
of where all the \(2\pi\)s belong), we list some properties of Fourier
transforms of general functions and probability densities in Facts
\ref{fact:fourier} and \ref{fact:gtwiddle}, respectively.

Finally, we will occasionally find it convenient to refer to
convolution and differentiation in operator notation, with \(T:
L_2(\mathbb{R}) \to L_2(\mathbb{R})\) mapping \(v \mapsto g*v\) and \(L: \mathcal{D}(L)
\subset L_2(\mathbb{R}) \to L_2(\mathbb{R})\) mapping \(v \mapsto v^{(2)}\).

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../JASA-template"
%%% End:


==> supplementalaux.tex <==


